PEFA: Parameter-Free Adapters for Large-scale Embedding-based Retrieval Models

Embedding-based Retrieval Models (ERMs) have emerged as a promising framework for large-scale text retrieval problems due to powerful large language models. Nevertheless, fine-tuning ERMs to reach state-of-the-art results can be expensive due to the extreme scale of data as well as the complexity of multi-stages pipelines (e.g., pre-training, fine-tuning, distillation). In this work, we propose the PEFA framework, namely ParamEter-Free Adapters, for fast tuning of ERMs without any backward pass in the optimization. At index building stage, PEFA equips the ERM with a non-parametric k-nearest neighbor (kNN) component. At inference stage, PEFA performs a convex combination of two scoring functions, one from the ERM and the other from the kNN. Based on the neighborhood definition, PEFA framework induces two realizations, namely PEFA-XL (i.e., extra large) using double ANN indices and PEFA-XS (i.e., extra small) using a single ANN index. Empirically, PEFA achieves significant improvement on two retrieval applications. For document retrieval, regarding Recall@100 metric, PEFA improves not only pre-trained ERMs on Trivia-QA by an average of 13.2%, but also fine-tuned ERMs on NQ-320K by an average of 5.5%, respectively. For product search, PEFA improves the Recall@100 of the fine-tuned ERMs by an average of 5.3% and 14.5%, for PEFA-XS and PEFA-XL, respectively. Our code is available at https://github.com/amzn/pecos/tree/mainline/examples/pefa-wsdm24.

==> tables/encoders.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\begin{tabular}{|l|l|rrrl|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{dataset}} & \multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{4}{c|}{Choice of Encoders}                                                                 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c}{TF-IDF} & \multicolumn{1}{c}{LaBSE} & \multicolumn{1}{c}{Sent-BERT} & TinyBERT(Prod) \\ \hline
\multirow{3}{*}{SM-7M}                         & ERM                                           & 3                          & 4                         & 5                             &                \\
                                               & ERM+FSI-XS                                    &                            &                           &                               &                \\
                                               & ERM+FSI-XL                                    &                            &                           &                               &                \\ \hline
\end{tabular}
\caption{Results of different encoders.}
\label{tab:exp-encoders}
\end{table*}

==> tables/main.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{l|l|rr|rrr|rr}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{dataset}} & \multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c|}{Evaluation Metrics}                           & \multicolumn{3}{c|}{Index Offline Building}                                                   & \multicolumn{2}{c}{Index Online Serving}                          \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c}{Recall@100} & \multicolumn{1}{c|}{Recall@1000} & \multicolumn{1}{c}{size (GBs)} & \multicolumn{1}{c}{GPU time} & \multicolumn{1}{c|}{CPU time} & \multicolumn{1}{c}{encoding} & \multicolumn{1}{l}{latency (ms/q)} \\

\midrule
\multirow{3}{*}{SM-7M}  & \ERM        & & & & & & & \\
                        & \ERM+\FSIxs & & & & & & & \\
                        & \ERM+\FSIxl & & & & & & & \\
\midrule
\multirow{3}{*}{SM-16M} & \ERM        & & & & & & & \\
                        & \ERM+\FSIxs & & & & & & & \\
                        & \ERM+\FSIxl & & & & & & & \\
\midrule
\multirow{3}{*}{SM-30M} & \ERM        & & & & & & & \\
                        & \ERM+\FSIxs & & & & & & & \\
                        & \ERM+\FSIxl & & & & & & & \\
\midrule
\multirow{3}{*}{SM-135M}& \ERM        & & & & & & & \\
                        & \ERM+\FSIxs & & & & & & & \\
                        & \ERM+\FSIxl & & & & & & & \\
\bottomrule
\end{tabular}%
}
\caption{main results}
\label{tab:exp-main}
\end{table*}
